Sinogram Enhancement with Generative Adversarial Networks using Shape Priors

Compensating scarce measurements by inferring them from computational models is a way to address ill-posed inverse problems. We tackle Limited Angle Tomography by completing the set of acquisitions using a generative model and prior-knowledge about the scanned object. Using a Generative Adversarial Network as model and Computer-Assisted Design data as shape prior, we demonstrate a quantitative and qualitative advantage of our technique over other state-of-the-art methods. Inferring a substantial number of consecutive missing measurements, we offer an alternative to other image inpainting techniques that fall short of providing a satisfying answer to our research question: can X-Ray exposition be reduced by using generative models to infer lacking measurements?

==> Sinogram Enhancement with Gans/sections/bibliography.tex <==
\begin{thebibliography}{00}

\bibitem{pathak2016context}Pathak, D., Krahenbuhl, P., Donahue, J., Darrell, T., \& Efros, A. A. "Context encoders: Feature learning by inpainting." Proceedings of the IEEE conference on computer vision and pattern recognition. 2016.

\bibitem{goodfellow2014generative}Goodfellow, I. J., Pouget-Abadie, J., Mirza, M., Xu, B., Warde-Farley, D., Ozair, S., ... \& Bengio, Y. "Generative adversarial nets." Advances in neural information processing systems. 2014. 

\bibitem{radford2015unsupervised}Radford, Alec, Luke Metz, and Soumith Chintala. "Unsupervised representation learning with deep convolutional generative adversarial networks." arXiv preprint arXiv:1511.06434 (2015).


\bibitem{yeh2016semantic} Yeh, Raymond A., et al. "Semantic image inpainting with deep generative models. ArXiv e-prints (2016)." arXiv preprint arXiv:1607.07539 (2016).

\bibitem{yoo2019sinogram} Yoo, Seunghwan, et al. "Sinogram Image Completion for Limited Angle Tomography With Generative Adversarial Networks." 2019 IEEE International Conference on Image Processing (ICIP). IEEE, 2019.

\bibitem{jahanian2019steerability}Jahanian, Ali, Lucy Chai, and Phillip Isola. "On the" steerability" of generative adversarial networks." arXiv preprint arXiv:1907.07171 (2019).

\bibitem{ronneberger2015u}Ronneberger, Olaf, Philipp Fischer, and Thomas Brox. "U-net: Convolutional networks for biomedical image segmentation." International Conference on Medical image computing and computer-assisted intervention. Springer, Cham, 2015.

\bibitem{isola2017image}Isola, P., Zhu, J. Y., Zhou, T., \& Efros, A. A. "Image-to-image translation with conditional adversarial networks." Proceedings of the IEEE conference on computer vision and pattern recognition. 2017.

\bibitem{ackerman1998visible}Ackerman, Michael J. "The visible human project." Proceedings of the IEEE 86.3 (1998): 504-511.

\bibitem{xu2007boundary}Xu, X. G., Taranenko, V., Zhang, J., \& Shi, C. "A boundary representation method for designing whole-body radiation dosimetry models: pregnant females at the ends of three gestational periods RPI P3, P6 and P9." Physics in Medicine \& Biology 52.23 (2007): 7023.

\bibitem{huang2013iterative}Huang, J., Zhang, Y., Ma, J., Zeng, D., Bian, Z., Niu, S., ... \& Chen, W. "Iterative image reconstruction for sparse-view CT using normal-dose image induced total variation prior." PloS one 8.11 (2013): e79709.

\bibitem{abbas2013super}Abbas, Sajid, Jonghwan Min, and Seungryong Cho. "Super-sparsely view-sampled cone-beam CT by incorporating prior data." Journal of X-ray science and technology 21.1 (2013): 71-83.

\bibitem{lee2018deep}Lee, H., Lee, J., Kim, H., Cho, B., \& Cho, S.  "Deep-neural-network-based sinogram synthesis for sparse-view CT image reconstruction." IEEE Transactions on Radiation and Plasma Medical Sciences 3.2 (2018): 109-119.



\bibitem{goodfellow2013maxout}Goodfellow, I., Warde-Farley, D., Mirza, M., Courville, A., \& Bengio, Y. (2013, May). Maxout networks. In International conference on machine learning (pp. 1319-1327). PMLR.


\bibitem{ioffe2015batch}Ioffe, Sergey, and Christian Szegedy. "Batch normalization: Accelerating deep network training by reducing internal covariate shift." arXiv preprint arXiv:1502.03167 (2015).

\bibitem{larsen2016autoencoding}Larsen, A. B. L., Sønderby, S. K., Larochelle, H., \& Winther, O. "Autoencoding beyond pixels using a learned similarity metric." International conference on machine learning. PMLR, 2016.

\bibitem{dupe2011inverse}Dupe, F-X., Mohamed-Jalal Fadili, and J-L. Starch. "Inverse problems with poisson noise: Primal and primal-dual splitting." 2011 18th IEEE International Conference on Image Processing. IEEE, 2011.

\bibitem{srivastava2014dropout} Srivastava, N., Hinton, G., Krizhevsky, A., Sutskever, I., \& Salakhutdinov, R "Dropout: a simple way to prevent neural networks from overfitting." The journal of machine learning research 15.1 (2014): 1929-1958.

\bibitem{nair2010rectified}Nair, Vinod, and Geoffrey E. Hinton. "Rectified linear units improve restricted boltzmann machines." ICML. 2010.

\bibitem{maas2013rectifier}Maas, Andrew L., Awni Y. Hannun, and Andrew Y. Ng. "Rectifier nonlinearities improve neural network acoustic models." Proc. icml. Vol. 30. No. 1. 2013.

\bibitem{coban2015sophiabeads_dataset}Coban, S. B., \& McDonald, S. A. (2015). SophiaBeads Dataset Project [Data set]. Zenodo. http://doi.org/10.5281/zenodo.16474

\bibitem{coban2015sophiabeads_codes}Coban, S. B. (2015, April 1). SophiaBeads Dataset Project Codes (Version v1.0). Zenodo. http://doi.org/10.5281/zenodo.16539

\bibitem{biguri2016tigre} Biguri, A., Dosanjh, M., Hancock, S., \& Soleimani, M. (2016). TIGRE: a MATLAB-GPU toolbox for CBCT image reconstruction. Biomedical Physics \& Engineering Express, 2(5), 055010.

\bibitem{ronchetti2020torchradon}Ronchetti, Matteo. "Torchradon: Fast differentiable routines for computed tomography." arXiv preprint arXiv:2009.14788 (2020).

\bibitem{jin2017deep}Jin, K. H., McCann, M. T., Froustey, E., \& Unser, M. "Deep convolutional neural network for inverse problems in imaging." IEEE Transactions on Image Processing 26.9 (2017): 4509-4522.

\bibitem{adler2017solving}Adler, Jonas, and Ozan Öktem. "Solving ill-posed inverse problems using iterative deep neural networks." Inverse Problems 33.12 (2017): 124007.

\bibitem{kelly2017deep}Kelly, Brendan, Thomas P. Matthews, and Mark A. Anastasio. "Deep learning-guided image reconstruction from incomplete data." arXiv preprint arXiv:1709.00584 (2017).

\bibitem{kingma2014Adam}Kingma, Diederik P., and Jimmy Ba. "Adam: A method for stochastic optimization." arXiv preprint arXiv:1412.6980 (2014).

\bibitem{goodfellow2016nips}Goodfellow, Ian. "NIPS 2016 tutorial: Generative adversarial networks." arXiv preprint arXiv:1701.00160 (2016).

\bibitem{sinha2020top}Sinha, S., Goyal, A., Raffel, C., \& Odena, A.  "Top-K Training of GANs: Improving Generators by Making Critics Less Critical." arXiv preprint arXiv:2002.06224 (2020).

\bibitem{valat2021codes} https://github.com/Emvlt/sinogram-interpolation-with-GAN

\bibitem{salimans2016improved}Salimans, T., Goodfellow, I., Zaremba, W., Cheung, V., Radford, A., \& Chen, X. "Improved techniques for training gans." arXiv preprint arXiv:1606.03498 (2016).

\end{thebibliography}

==> Sinogram Enhancement with Gans/sections/commands.tex <==
\newcommand{\xr}{X-Ray }
\newcommand{\xrs}{X-Rays }
